Marginalized Importance Sampling for Off-Environment Policy Evaluation

Reinforcement Learning (RL) methods are typically sample-inefficient, making it challenging to train and deploy RL-policies in real world robots. Even a robust policy trained in simulation requires a real-world deployment to assess their performance. This paper proposes a new approach to evaluate the real-world performance of agent policies prior to deploying them in the real world. Our approach incorporates a simulator along with real-world offline data to evaluate the performance of any policy using the framework of Marginalized Importance Sampling (MIS). Existing MIS methods face two challenges: (1) large density ratios that deviate from a reasonable range and (2) indirect supervision, where the ratio needs to be inferred indirectly, thus exacerbating estimation error. Our approach addresses these challenges by introducing the target policy's occupancy in the simulator as an intermediate variable and learning the density ratio as the product of two terms that can be learned separately. The first term is learned with direct supervision and the second term has a small magnitude, thus making it computationally efficient. We analyze the sample complexity as well as error propagation of our two step-procedure. Furthermore, we empirically evaluate our approach on Sim2Sim environments such as Cartpole, Reacher, and Half-Cheetah. Our results show that our method generalizes well across a variety of Sim2Sim gap, target policies and offline data collection policies. We also demonstrate the performance of our algorithm on a Sim2Real task of validating the performance of a 7 DoF robotic arm using offline data along with the Gazebo simulator.

==> outline/LearningQ.tex <==
\section{Learning Q Function}

==> outline/dice_version.tex <==
\section{DICE version of Off Environment Evaluation}
Consider the following optimization 
\begin{align*}
   \min_{x} J(x) = \frac{1}{2} \EE_{(s, a) \sim d^{\pi}_{\tr}} [x(s, a)^2] - \EE_{(s, a) \sim d^{\pi}_{\te}} [x(s, a)]
\end{align*}
We can substitute $v(s, a) - \gamma \EE_{s' \sim \te(\cdot | s, a), a' \sim \pi(\cdot | s')}[v(s', a')] = x(s, a)$. We thus get the following optimization 
\begin{align}
    \frac{1}{2} \EE_{(s, a) \sim d^{\pi}_{\tr}} [(v(s, a) - \gamma \EE_{s' \sim \te(\cdot | s, a), a' \sim \pi(\cdot | s')}[v(s', a')])^2] - (1 - \gamma) \EE_{s \sim d_0, a \sim \pi(\cdot | s)} [v(s, a)]
\end{align}
Following the derivation procedure by substituting the dual formulation in the first term. We get the following 
\begin{align*}
    &\min_x \max_{\zeta} J(x, \zeta) = \underbrace{\EE_{(s, a) \sim d^{\pi}_{\tr}}[(v(s, a) - \gamma \EE_{s' \sim \te(\cdot | s, a), a' \sim \pi(\cdot | s')}[v(s', a')])\cdot \zeta(s, a) - \frac{1}{2} \zeta(s, a)^2]}_{\textbf{first term}} \\
     &- (1 - \gamma) \EE_{s \sim d_0, a \sim \pi(\cdot | s)} [v(s, a)]
\end{align*}
Let's concentrate on the first term here. 
\begin{align*}
    &= \EE_{(s, a) \sim d^{\pi}_{\tr}}[(v(s, a) - \gamma \EE_{s' \sim \te(\cdot | s, a), a' \sim \pi(\cdot | s')}[v(s', a')])\cdot \zeta(s, a) - \frac{1}{2} \zeta(s, a)^2] \\
    &= \EE_{(s, a) \sim d^{\pi}_{\tr}}[(v(s, a) - \gamma \EE_{s' \sim \tr(\cdot | s, a), a' \sim \pi(\cdot | s')}[v(s', a')] + \gamma \EE_{s' \sim \tr(\cdot | s, a), a' \sim \pi(\cdot | s')}[v(s', a')] - \gamma \EE_{s' \sim \te(\cdot | s, a), a' \sim \pi(\cdot | s')}[v(s', a')])\cdot \zeta(s, a)] \\
    &\EE_{(s, a) \sim d^{\pi}_{\tr}}[(v(s, a) - \gamma \EE_{s' \sim \tr(\cdot | s, a), a' \sim \pi(\cdot | s')}[v(s', a')])\cdot \zeta(s, a)] \\
    &+ \gamma \EE_{(s, a) \sim d^{\pi}_{\tr}}[(\EE_{s' \sim \tr(\cdot | s, a), a' \sim \pi(\cdot | s')}[v(s' , a')] -\EE_{s' \sim \te(\cdot | s, a), a' \sim \pi(\cdot | s')}[v(s' , a')]) \cdot \zeta(s, a)]
\end{align*}

==> outline/introduction_alternate.tex <==
\section{Introduction}
Offline Reinforcement learning (RL) has recently gained much popularity for their ability to train robots using fixed batch of data \cite{levine2020offline}. An important aspect in Offline RL includes constantly re-evaluating performance of learned policies over the course of training. Off Policy Evaluation (OPE) are one-class of methods that use data collected from \textit{behavior} policy to estimate the performance of a different \textit{target} policy. 

Classical OPE methods are based on the principle of importance sampling (IS) \cite{precup2000eligibility, jiang2016doubly}, which reweights each trajectory by its density ratio under the target vs.~the behavior policies. Despite being unbiased, IS  suffers exponential-in-horizon variance when the target policy deviates significantly from the behavior policy. More recently, significant progress has been made on \textit{marginzed importance sampling} (MIS), which reweights transition tuples using the density ratio (or importance weights) over states instead of trajectories to overcome the so-called curse of horizon \cite{liu2018breaking, nachum2020reinforcement, uehara2019minimax}. The density ratio in this case, however, cannot be calculated directly as in IS, and often needs to be learned via optimizing minimax loss functions. In most existing MIS methods are model-free, relying on data from the real environment and function approximators of value and weight functions. 

In applications such as robotics, however, it is reasonable to assume access to a good but possibly imperfect model/simulator of the real environment, and we investigate how to improve MIS methods using such a simulator as side information. In particular, the weight-estimation procedure in existing model-free MIS methods face two difficulties \textit{simultaneously}, that:
\begin{enumerate}[leftmargin=*]
\item \textit{Large ratios:} the weight function corrects the distribution mismatch between the behavior and the target policies and thus needs to deviate significantly from $1$, which can be challenging to learn. 
\item \textit{Indirect supervision:} no samples from the target policies' occupancy are available, and the weight needs to be inferred \textit{indirectly} via the Bellman flow equation using difficult minimax optimization. 
\end{enumerate}
In this paper, we propose a new MIS method that addresses the above challenges with the help of a good but imperfect simulator. By introducing the target policy's occupancy \textit{in the simulator} as an intermediate variable, our method splits the weight to be learned into the product of two terms and learns them separately, where the first term enjoys \textit{direct supervision} and the second term has \textit{small magnitude} (i.e., close to 1). We provide a simple derivation of our method, analyze its theoretical properties, and compare it to baselines empirically (including existing ways of incorporating a simulator in OPE). More concretely, our contributions are 3-fold:
%Off-policy evaluation (OPE) is the problem of using data collected from a \textit{behavior} policy to estimate the performance of a different \textit{target} policy, and plays an important role in the pipeline of offline reinforcement learning (RL) for real-world applications \cite{levine2020offline}. Most existing OPE methods are model-free, relying on data from the real environment and function approximators of value and (sometimes) importance-weight (or density-ratio) functions. In applications such as robotics, however, it is reasonable to assume access to a good but possibly imperfect model/simulator of the real environment. Based on this observation, we investigate how to use such a simulator as side information to improve the accuracy of MIS. In particular, we wish to address a challenge in existing MIS methods, that they face the following two difficulties \textit{simultaneously}:
%\begin{enumerate}[leftmargin=*]
%\item \textit{Large ratios:} the weight function corrects the distribution mismatch between the behavior and the target policies and thus needs to deviate significantly from $1$, which can be challenging to learn. 
%\item \textit{Indirect supervision:} no samples from the target policies' occupancy are available, and the weight needs to be inferred \textit{indirectly} via the Bellman flow equation using difficult minimax optimization. 
%\end{enumerate}
%In this paper, we propose a new MIS method that addresses the above challenges with the help of a good but imperfect simulator. By introducing the target policy's occupancy \textit{in the simulator} as an intermediate variable, our method splits the weight to be learned into the product of two terms and learns them separately, where the first term enjoys \textit{direct supervision} and the second term has \textit{small magnitude}. We provide a simple derivation of our method, analyze its theoretical properties, and compare it to related works including existing ways of incorporating a simulator in OPE. Our contributions are three-fold:
\begin{enumerate}
\item We derive an MIS estimator for off-environment evaluation (Section~\ref{sec:weight estimator})
\item We analyze the theoretical properties of our estimator by a general sample-complexity analysis (Section~ \ref{sec:guarantee}) and studying its special cases in linear and kernel settings.
\item We empirically evaluate  our estimator on Sim2Sim environments like Cartpole and Halfcheetah and compare it to other baselines that use the real data and/or the imperfect simulator. We also explore practicality of this estimator by evaluating over a Sim2Real problem of validating performance of a kinova gen3 robot using its simulator.  (Section~\ref{sec:experiment}).
\end{enumerate}

==> outline/relatedwork.tex <==
\section{Related Works}
We review related works in this section, focusing on comparing to existing OPE methods that can leverage the side information provided by an imperfect simulator.

\paragraph{Doubly Robust estimators} In the importance sampling (IS) family, doubly robust (DR) estimators \citep{jiang2016doubly, thomas2016data} incorporate approximate Q-functions as control variates for variance reduction. When a simulator is available, we can compute Q-functions from the simulator as such control variates. However, this cannot fully address the exponential variance issue of IS estimators, as the variance of IS due to stochastic transitions and imperfect control variates will still be blown up by the cumulative importance weights \citep{jiang2016doubly}.

\paragraph{MIS estimators} As mentioned in the introduction, most MIS methods are model-free. Similar to DR for IS, \citet{uehara2019minimax, tang2019doubly} show that MIS estimators also have a DR form and can benefit from Q-functions as control variates, which can be supplied by the simulator. However, the DR version of MIS is a meta estimator, and the weight $d_{\te}^\pi/\mu$ still needs to be estimated via a ``base'' MIS procedure. Therefore, our estimator can also benefit from the DR form, and the simulator will reduce the variance in two independent ways that do not conflict with each other: the simulator makes the estimation of $d_{\te}^\pi/\mu = \beta \cdot \wpp$ easier, and also improves the variance of the final estimator $\EE_{\mu}[d_{\te}^\pi/\mu \cdot r]$ via additionally supplying a Q-function as control variate. 
\paragraph{MML \citep{voloshin2021minimax}} The work of \citet{voloshin2021minimax} considers model-based OPE and is strongly inspired by MIS. However, the work is different from ours in several ways: first, \citet{voloshin2021minimax} learns a model from a \textit{model class}, and directly outputs the prediction from the learned model for OPE. As a result, the success of their method relies on the well-specification of the model class. In comparison, we only have a single simulator, and our guarantee in Theorem~\ref{thm:finite-sample} does \textit{not} rely on the simulator being accurate; the simulator only provides auxiliary variables $d_{\tr}^\pi$ to facilitate learning. Second, while \citet{voloshin2021minimax} is motivated by ``decision-aware'' model learning, their learning procedure is still relatively generic, and the awareness of the OPE task is only reflected in the analysis through the realizability assumptions of the function classes, and it is difficult to adapt the algorithm to specific OPE tasks in practice. In contrast, our method explicitly extracts information about the target policy $\pi$ from the simulator, and is explicitly tuned towards the evaluation of policy $\pi$ in a straightforward manner.

==> outline/reviews.tex <==
\onecolumn 
\section{Reviews}
\subsection{Reviewer 1}
Dear Reviewer 6c7d,

Thank you for your comments and appreciation of `the paper’s high-level intuition' and our `novel decomposition'. We also agree with your evaluation about the limitations of the paper and will improve accordingly in revision (e.g., more combinations of dynamics/policy shift). 

In your reviews you mentioned end-to-end analyses/learning. We believe some clarifications can help you better understand the nature of our results, and will focus our response to this point. 

\begin{enumerate}
    \item \textit{The bound is claimed to be end-to-end. But how the error of $\beta$ should affect the ultimate result is not clear. The bound still depends on the estimated $\beta$}

Thanks for pointing out that our bound still depends on the estimated $\beta$! Concretely, this is reflected in the $\min_w \max_q L_w(w, \hat\beta, q)$ term in both bounds of Theorem 6. \\
We actually have 2 versions of this theorem (one of which doesn’t depend on $\hat \beta$), and accidentally put the $\hat\beta$ version in the submission; really sorry about the confusion and we will fix that. The version without $\hat\beta$ is actually very easy to obtain from what we have in the submission: from the error decomposition on pg 13 (see the multi-line eq above Eq.27), we have $\min_w \max_q |L_w(w, \hat\beta, q)|$ as the very last term, which is why you see it in the theorem statement. To get rid of it,

$\min_{w \in \Wcal} \max_{q \in \Qcal} |L_w(w, \hat\beta, q)|$
$ \le \max_{q \in \Qcal} |L_w(w_{P/P’}^\pi, \hat \beta, q)|$ (relax $\min_w$ to true $w$)\\
$ = \max_{q \in \Qcal} |L_w(w_{P/P’}^\pi, \frac{d^\pi_{\tr}}{\mu}, q)| +   \max_{q \in \Qcal} |L_w(w_{P/P’}^\pi, \hat \beta, q)| -  \max_{q \in \Qcal} |L_w(w_{P/P’}^\pi, \frac{d^\pi_{\tr}}{\mu}, q)|$ (true $w$ & true $\beta$ have 0 population loss)\\
$ \le  \max_{q \in \Qcal} |L_w(w_{P/P’}^\pi, \frac{d^\pi_{\tr}}{\mu}, q)| + \underbrace{\max_{q \in \Qcal}|L_w(w_{P/P’}^\pi, \hat \beta, q) - L_w(w_{P/P’}^\pi, \frac{d^\pi_{\tr}}{\mu}, q)|}_{T_2}$ (diff between max is bounded by max over diff)

The final error term here is basically the $T_2$ term in our proof, with the only difference that $T_2$ has $\hat w$ and here we have true $w$. Furthermore, we didn’t use any special properties of $\hat w$ when bounding $T_2$, so exactly the same bound applies to the above quantity. As a result, we can drop the $\hat\beta$ term in Theorem 6 and the rest of the error bounds will blow up by only a constant factor (and hence absorbed by $O(\cdot)$). 

\item \textit{Considering … how the two components (off-dynamics and off-policy) may affect each other, a more interesting thing to consider is how to learn [$\beta$ and $w$] together}

1. We agree it would be desirable to learn $\beta$ and $w$ jointly, though it is unclear how to do it. In our current formulation, $\beta$ and $w$ are learned using very different loss functions, which cannot be easily combined. 

2. That said, we argue that a major benefit of joint learning is the robustness against misspecification, and failure of a single component can be compensated by other components. To that end, our current method already partially enjoys this property. The key is that the two stages of our algorithm are not independent of each other, and the second stage of learning $w$ actually uses the $\hat\beta$ learned in the first stage. If the function class for $w$ is sufficiently rich, it can possibly make up for the large errors made in the first stage. 

Concretely, suppose $\hat{\beta}$ learned in the first stage is a very poor approximation of the true $\beta$, possibly because the function class $\mathcal{F}$ for learning $\beta$ is misspecified. Then, as long as $\mathcal{W}$ is sufficiently rich to capture $w_P^{\pi/\mu} / \hat\beta$ (note that this coincides with our realizability assumption when $\hat \beta = \frac{d^\pi_{\tr}}{\mu})$, we will still enjoy provable guarantees, as the second stage can learn $w \approx w_P^{\pi/\mu} / \hat\beta$ to “compensate” for the error in $\hat \beta$. (We didn’t include this result because the realizability of $w_P^{\pi/\mu} / \hat\beta$ is not an “a priori” assumption since it depends on data randomness, which is considered undesirable in ML theory; the proof is also more straightforward and less challenging. Plus, $w_P^{\pi/\mu} / \hat\beta$ may not have magnitude close to 1 and some of the benefits of our approach are lost.) We will add discussions in the paper.

We also thought about demonstrating this effect empirically by an ablation study. Concretely, if we could have access to the true $\beta$, we could use it in the second stage of learning $w$, and combine the learned $w$ with the learned $\beta$ in the final prediction. This way, the two stages are completely independent of each other, and the hypothesis is that this is worse than our algorithm. The difficulty in empirical evaluation of this idea is that it is very difficult to compute true density ratios in realistic problems with large state spaces. We are thinking about alternative ways of demonstrating this empirically and will add the results to the revision if we have a good plan.
\end{enumerate}
\subsection{Reviewer 2}
Dear Reviewer dAXy,

Thank you for your comments that the paper is easy to understand and the proposed method is well motivated. We also agree with your evaluation about the limitations of the paper and will improve accordingly in revision. Below we respond to your technical questions:

\begin{enumerate}
    \item \textit{Can you provide the rigorous proof of Eq (6)? }
    
    The first step of Eq.6 directly follows from the definition of $w_{P/P’}^\pi$ and the principle of importance sampling, which is fundamental to all of IS/MIS works. I.e., $w_{P/P’}^\pi$ is defined as the density ratio between $d_{P}^\pi$ and $d_{P’}^\pi$, so the change of measure directly follows. The second step follows directly from the bellman flow equation, as we commented in the text below the equation. For a proof, see Lemma 3 of Liu et al (\href{https://arxiv.org/pdf/1810.12429.pdf}{https://arxiv.org/pdf/1810.12429.pdf}). The Bellman flow equation specifies the temporal consistency of discounted occupancies, just as the usual Bellman equation specifies the temporal consistency of value functions. From an LP duality perspective of MDPs, these two equations are often treated “symmetrically”. And just like we often omit the proof for the usual Bellman equation of value functions, here we skip its proof in this derivation where the main purpose is to provide intuitions. 
    \item \textit{In what cases the sample complexity of the proposed method could be superior to traditional MIS that bears the two difficulties simultaneously?}
    
    The improvement is not directly shown in the theorem statement, and rather nuanced. For example, because our $\mathcal{W}$ class only needs to model the “off-environment” shift $w_{P/P’}^\pi$ ($\approx 1$ when $P \approx P’$), the magnitude of the functions in $\mathcal{W}$ (i.e., the constant $C_{\mathcal{W}}$) can be set relatively small when we design the function class. This does not directly reflect as an improvement in the sample complexity bound as $C_{\mathcal{W}}$ is multiplied by $C_{\mathcal{F}}$ in the bound, where $C_{\mathcal{F}}$ depends on the magnitude of “off-policy” shift and can be large. However, working with functions with small magnitude can be helpful in difficult minimax optimization (which is required in our 2nd stage of learning $w$ as well as virtually all DICE-style algorithms), which can easily run into instability issues. Overall, we agree with the criticism that the improvement is not directly shown by the theorems, likely due to the worst-case nature of these bounds, but we hope the paper has provided good intuitions for why the idea can be useful. 
\end{enumerate}



\subsection{Reviewer 3}
Dear Reviewer Jvmh,

Thank you for your comments. We will add more discussions and interpretations of the theoretical results, especially based on the questions being asked by the review team.

